Uncertainty Estimation in SARS-CoV-2 B-cell Epitope Prediction for Vaccine Development

B-cell epitopes play a key role in stimulating B-cells, triggering the primary immune response which results in antibody production as well as the establishment of long-term immunity in the form of memory cells. Consequently, being able to accurately predict appropriate linear B-cell epitope regions would pave the way for the development of new protein-based vaccines. Knowing how much confidence there is in a prediction is also essential for gaining clinicians' trust in the technology. In this article, we propose a calibrated uncertainty estimation in deep learning to approximate variational Bayesian inference using MC-DropWeights to predict epitope regions using the data from the immune epitope database. Having applied this onto SARS-CoV-2, it can more reliably predict B-cell epitopes than standard methods. This will be able to identify safe and effective vaccine candidates against Covid-19.

==> bibliography.tex <==
@article{mak2014b,
  title={B cell development, activation and effector functions},
  author={Mak, TW and Saunders, ME and Jett, BD},
  journal={Primer to the immune response. 2nd ed: Academic Cell},
  pages={111--42},
  year={2014}
}
@article{blythe2005benchmarking,
  title={Benchmarking B cell epitope prediction: underperformance of existing methods},
  author={Blythe, Martin J and Flower, Darren R},
  journal={Protein Science},
  volume={14},
  number={1},
  pages={246--248},
  year={2005},
  publisher={Wiley Online Library}
}
@article{janeway2001immune,
  title={The immune system in health and disease},
  author={Janeway, Charles A},
  journal={http://www. garlandscience. com},
  year={2001}
}
@article{sanchez2017fundamentals,
  title={Fundamentals and methods for T-and B-cell epitope prediction},
  author={Sanchez-Trincado, Jose L and Gomez-Perosanz, Marta and Reche, Pedro A},
  journal={Journal of immunology research},
  volume={2017},
  year={2017},
  publisher={Hindawi}
}

@article{hopp1981prediction,
  title={Prediction of protein antigenic determinants from amino acid sequences},
  author={Hopp, Thomas P and Woods, Kenneth R},
  journal={Proceedings of the National Academy of Sciences},
  volume={78},
  number={6},
  pages={3824--3828},
  year={1981},
  publisher={National Acad Sciences}
}
@article{hopp1983computer,
  title={A computer program for predicting protein antigenic determinants},
  author={Hopp, Thomas P and Woods, Kenneth R},
  journal={Molecular immunology},
  volume={20},
  number={4},
  pages={483--489},
  year={1983},
  publisher={Elsevier}
}

@article{lins2003analysis,
  title={Analysis of accessible surface of residues in proteins},
  author={Lins, Laurence and Thomas, Annick and Brasseur, Robert},
  journal={Protein science},
  volume={12},
  number={7},
  pages={1406--1417},
  year={2003},
  publisher={Wiley Online Library}
}

@article{b1,
    author =       "D. A. V. Valen and T. Kudo and K. M. Lane and D. N. Macklin and N. T. Quach and M. M. DeFelice and I. Maayan and Y. Tanouchi and E. A. Ashley and M. W. Covert",
    title =        "Deep learning automates the quantitative analysis of individual cells in live-cell imaging experiments",
    journal =      "PLOS Computational Biology",
    volume =       "12(11):e1005177",
    number =       "",
    pages =        "",
    year =         "nov 2016",
    DOI =          ""
}

@article{nomi2020epitope,
  title={Epitope Prediction of Antigen Protein using Attention-Based LSTM Network},
  author={Nomi, Toshiaki and Inoue, Seiichi and Fujita, Haruka and Sadamitsu, Kugatsu and Sakaguchi, Makoto and Tenma, Akiko and Nakagami, Hironori},
  journal={BioRxiv},
  year={2020},
  publisher={Cold Spring Harbor Laboratory}
}

@article{ghoshal2020estimating_ci,
  title={Estimating uncertainty in deep learning for reporting confidence to clinicians in medical image segmentation and diseases detection},
  author={Ghoshal, Biraja and Tucker, Allan and Sanghera, Bal and Lup Wong, Wai},
  journal={Computational Intelligence},
  publisher={Wiley Online Library}
}
@article{ghoshal2020estimating_covid,
  title={Estimating uncertainty and interpretability in deep learning for coronavirus (COVID-19) detection},
  author={Ghoshal, Biraja and Tucker, Allan},
  journal={arXiv preprint arXiv:2003.10769},
  year={2020}
}

@article{Kaggle,
    author =       "",
    title =        "",
    journal =      "COVID-19/SARS B-cell Epitope Prediction",
    volume =       "",
    number =       "",
    pages =        "",
    year =         "2019",
    url =          "https://www.kaggle.com/c/data-science-bowl2018"
}

@article{Blundell,
    author =       "C. Blundell and J. Cornebise and K. Kavukcuoglu and D. Wierstra",
    title =        "Weight uncertainty in neural networks",
    journal =      "arXiv preprint arXiv:1505.05424",
    volume =       "",
    number =       "",
    pages =        "",
    year =         "2015",
    DOI =          ""
}

@article{Kwon,
    author =       "Kwon, Y. and Won, J.-H. and Kim, B. J. and Paik, M. C.",
    title =        "Uncertainty quantification using bayesian neural networks in classification: Application to ischemic stroke lesion segmentation",
    journal =      "Medical Imaging with Deep Learning Conference",
    volume =       "",
    number =       "",
    pages =        "",
    year =         "2018",
    DOI =          ""
}

@article{Gal,
    author =       "Gal, Y and Ghahramani, Z",
    title =        "Dropout as a Bayesian approximation: Representing model uncertainty in deep learning",
    journal =      "33rd International Conference on Machine Learning, ICML 2016, 3",
    volume =       "",
    number =       "",
    pages =        "1651-1660",
    year =         "2016",
    DOI =          ""
}

@article{Gal_Thesis,
    author =       "Yarin Gal",
    title =        "Uncertainty in Deep Learning",
    journal =      "PhD thesis, University of Cambridge",
    volume =       "",
    number =       "",
    pages =        "",
    year =         "2016",
    DOI =          ""
}

@article{Kendall,
    author =       "Alex Kendall and Yarin Gal",
    title =        "What uncertainties do we need in bayesian deep learning for computer vision?",
    journal =      "In Advances in Neural Information Processing Systems",
    volume =       "",
    number =       "",
    pages =        "5580-5590",
    year =         "2017",
    DOI =          ""
}

@article{MacKay,
    author =       "David JC MacKay",
    title =        "A practical bayesian framework for backpropagation networks",
    journal =      "Neural computation",
    volume =       "4(3):448-472",
    number =       "",
    pages =        "",
    year =         "1992",
    DOI =          ""
}

@article{Neal,
    author =       "Radford M Neal",
    title =        "Bayesian learning via stochastic dynamics",
    journal =      "In Advances in neural information processing systems",
    volume =       "",
    number =       "",
    pages =        "475-482",
    year =         "1993",
    DOI =          ""
}

@article{Goodfellow,
    author =       "Ian Goodfellow and Yoshua Bengio and Aaron Courville",
    title =        "Deep learning",
    journal =      "MIT press Cambridge",
    volume =       "1",
    number =       "",
    pages =        "",
    year =         "2016",
    DOI =          ""
}
@inproceedings{lacoste2011approximate,
  title={Approximate inference for the loss-calibrated Bayesian},
  author={Lacoste--Julien, Simon and Husz{\'a}r, Ferenc and Ghahramani, Zoubin},
  booktitle={Proceedings of the Fourteenth International Conference on Artificial Intelligence and Statistics},
  pages={416--424},
  year={2011}
}
@article{cobb2018loss,
  title={Loss-calibrated approximate inference in Bayesian neural networks},
  author={Cobb, Adam D and Roberts, Stephen J and Gal, Yarin},
  journal={arXiv preprint arXiv:1805.03901},
  year={2018}
}
